Multiple Receiver Over-the-Air Computation for Wireless Networked Control Systems

We propose a multi-sender, multi-receiver over-the-air computation (OAC) framework for wireless networked control systems (WNCS) with structural constraints. Our approach enables actuators to directly compute and apply control signals from sensor measurements, eliminating the need for a centralized controller. We use an iterative and convexifying procedure to obtain a control law that is structured with respect to the network topology and minimizes the overall system energy-to-energy gain. Furthermore, we solve a constrained matrix factorization problem to find the optimal OAC configuration with respect to power consumption, robustness, and stability of the WNCS. We prove the convergence of our proposed algorithms and present numerical results that validate our approach to preserve closed-loop stability with robust control performance and constrained power.

==> Figures/Topology21.tex <==
\begin{figure}[t!]
    \centering
















\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-0.75,xscale=0.75]
%uncomment if require: \path (0,392); %set diagram left start at 0, and has height of 392


%Straight Lines [id:da38391948833277745] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (259.33,104) -- (366,104.98) ;
\draw [shift={(368,105)}, rotate = 180.53] [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da4552473623228146] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (261.33,156) -- (367,155.02) ;
\draw [shift={(369,155)}, rotate = 179.47] [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da46496367564530794] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ]   (263.33,255) -- (272,254.36) -- (367,254.99) ;
\draw [shift={(369,255)}, rotate = 180.38] [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da22797866883741258] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ]   (263.33,255) -- (367.55,156.37) ;
\draw [shift={(369,155)}, rotate = 136.58] [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da5665365381913907] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (259.33,104) -- (367.82,253.38) ;
\draw [shift={(369,255)}, rotate = 234.01] [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da204250087802476] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (261.33,156) -- (366.2,105.86) ;
\draw [shift={(368,105)}, rotate = 154.45] [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Curve Lines [id:da18610836687286314] 
\draw    (362.33,123) .. controls (355.51,125.93) and (328.72,106.03) .. (345.92,91.14) ;
\draw [shift={(347.33,90)}, rotate = 143.13] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Curve Lines [id:da04836356985167556] 
\draw    (359.33,176) .. controls (352.51,178.93) and (325.72,159.03) .. (342.92,144.14) ;
\draw [shift={(344.33,143)}, rotate = 143.13] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Curve Lines [id:da9621176276124825] 
\draw    (351.33,262) .. controls (346.18,264.69) and (338.72,232.67) .. (358.74,219.94) ;
\draw [shift={(360.33,219)}, rotate = 151.39] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Rectangle [id:dp7857217760380266] 
\draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ] (580.68,142.14) -- (579.83,210.51) -- (424.29,208.59) -- (425.14,140.21) -- cycle ;
%Straight Lines [id:da8117517075778167] 
\draw    (387,106) -- (436.33,106) ;
%Straight Lines [id:da5670422380318003] 
\draw    (436.33,106) -- (436.33,138) ;
\draw [shift={(436.33,141)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da9680065060740795] 
\draw    (390.33,156) -- (422.33,156) ;
\draw [shift={(425.33,156)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da5283214230131499] 
\draw    (394.33,254) -- (440.33,254) ;
%Straight Lines [id:da03917255663299146] 
\draw    (440.33,211) -- (440.33,254) ;
\draw [shift={(440.33,208)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da24966496869479848] 
\draw    (461,209) -- (460.2,270.6) ;
%Straight Lines [id:da052875854359592855] 
\draw    (471.2,209.6) -- (471.2,280.6) ;
%Straight Lines [id:da6759055925320168] 
\draw    (220.2,279.6) -- (471.2,280.6) ;
%Straight Lines [id:da6037082797486906] 
\draw    (230,257) -- (244,257) ;
\draw [shift={(247,257)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da5432710152934956] 
\draw    (230.2,271.6) -- (460.2,270.6) ;
%Straight Lines [id:da34569258006707915] 
\draw    (230,257) -- (230.2,271.6) ;
%Straight Lines [id:da8387858484716904] 
\draw    (219.2,155.6) -- (220.2,279.6) ;
%Straight Lines [id:da2103870246143391] 
\draw    (219.2,155.6) -- (237.2,155.6) ;
\draw [shift={(240.2,155.6)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da6343780831389967] 
\draw    (209.67,104.67) -- (209.2,288.6) ;
%Straight Lines [id:da7782464342243063] 
\draw    (209.2,288.6) -- (481.2,289.6) ;
%Straight Lines [id:da623352570772832] 
\draw    (481.2,289.6) -- (481.2,209.6) ;
%Straight Lines [id:da756830967077575] 
\draw    (209.67,104.67) -- (233.2,104.61) ;
\draw [shift={(236.2,104.6)}, rotate = 179.86] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;

% Text Node
\draw (244.2,94) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {$\displaystyle s_{1}$};
% Text Node
\draw (245.2,144) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {$\displaystyle s_{2}$};
% Text Node
\draw (249.2,245) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {$\displaystyle s_{p}$};
% Text Node
\draw (371.67,95.67) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {$\displaystyle a_{1}$};
% Text Node
\draw (372.2,145) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {$\displaystyle a_{2}$};
% Text Node
\draw (242.01,183) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \vdots $};
% Text Node
\draw (369.67,183) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \vdots $};
% Text Node
\draw (373.2,244) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {$\displaystyle a_{m}$};
% Text Node
\draw (337,70.4) node [anchor=north west][inner sep=0.75pt]    {$\mathcal{N}_{a}{}_{_{1}}$};
% Text Node
\draw (334,123.4) node [anchor=north west][inner sep=0.75pt]    {$\mathcal{N}_{a}{}_{_{2}}$};
% Text Node
\draw (341,194.4) node [anchor=north west][inner sep=0.75pt]    {$\mathcal{N}_{a}{}_{_{m}}$};
% Text Node
\draw (486,143) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textbf{Plant}};
% Text Node
\draw (427.33,159.4) node [anchor=north west][inner sep=0.75pt]    {\tiny$\mathbf{x}[ k+1] \ =\ \mathbf{Ax}[ k] \ +\mathbf{Bu}[ k] \ $};
% Text Node
\draw (453.33,177.4) node [anchor=north west][inner sep=0.75pt]    {\tiny$\mathbf{y}[ k] \ =\ \mathbf{Cx}[ k]$};


\end{tikzpicture}



\caption{Caption}
\label{fig:enter-label}
\end{figure}

==> Figures/Topology_copy.tex <==
\definecolor{sage}{HTML}{57d491}
\definecolor{niceblue}{HTML}{57a8d4}

\begin{figure}[t!]
\centering
\begin{tikzpicture}[transform shape, scale=1,thick]
\tikzstyle{every node}=[font=\footnotesize]
    % \node at (4.3,2.8) {\footnotesize Map};
    % \draw[thick] [decorate, decoration = {brace}] (3.4,2.5) --  (5.2,2.5);
    
    % \node at (5.95,2.8) {\footnotesize Shuffle};
    % \draw[thick] [decorate, decoration = {brace}] (5.3,2.5) --  (6.6,2.5);
    % \node at (7.55,2.8) {\footnotesize Reduce};
    % \draw[thick] [decorate, decoration = {brace}] (6.7,2.5) --  (8.4,2.5);
    
    % \foreach \x/\y in {1.45/1,0.35/2,-1.25/$K$}%{1,2,3,4,5,6,7,8}
    %     \draw[fill=sage,rounded corners] (3.5,\x-0.15) rectangle node[black] {\y} ++(0.6,0.6);
    % \node at (3.8,-0.3) {$ \vdots$};

    % \draw[->] (2.6,1.75-0.15) -- (3.5,1.75-0.15);
    % \draw[->] (2.6,0.65-0.15) -- (3.5,0.65-0.15);
    % \draw[->] (2.6,-0.95-0.15) -- (3.5,-0.95-0.15);
    \foreach \x/\y in {1.75/1,0.65/2,-0.95/p}
        \node at (5,\x-0.15) {$s_\y$};
    \node at (5,-0.3) {$ \vdots$};
    % \draw[->] (4.1,1.75-0.15) -- (4.75,1.75-0.15);
    % \draw[->] (4.1,0.65-0.15) -- (4.75,0.65-0.15);
    % \draw[->] (4.1,-0.95-0.15) -- (4.75,-0.95-0.15);

    %\draw[->] (5.3,1.75) -- (6.5,1.75) node [midway,above] {\footnotesize $d_{q,1}$};
    %\draw[->] (5.3,0.65) -- (6.5,0.65) node [midway,above] {\footnotesize $d_{q,2}$};
    %\draw[->] (5.3,-0.95) -- (6.5,-0.95) node [midway,above] {\footnotesize $d_{q,K}$};
    \filldraw[blue] (5.4,1.75-0.15) circle (1.5pt);
    \draw[->,blue] (5.4,1.75-0.15) -- (6.6,1.75-0.15);
    \draw[->,blue] (5.4,1.75-0.15) -- (6.6,0.65-0.15);
    \draw[->,blue] (5.4,1.75-0.15) -- (6.6,-0.95-0.15);
    %\draw[->,thick,dotted] (5.2,1.3) .. controls +(down:0.8) and +(right:0.9) .. (6,2) node[anchor=east]{$\mathcal{T}_1$};
    \draw[->,dashed] (5.2,1.3-0.15) .. controls (5.8,1.5-0.15) .. (6,2-0.15);
    \node[] at (6,2.1) {\scriptsize$\mathcal{N}_{s_1}$};
    
    \filldraw[cyan] (5.4,0.65-0.15) circle (1.5pt);
    \draw[->,cyan] (5.4,0.65-0.15) -- (6.6,0.65-0.15);
    \draw[->,cyan] (5.4,0.65-0.15) -- (6.6,1.75-0.15);
    \draw[->,cyan] (5.4,0.65-0.15) -- (6.6,-0.95-0.15);

    \filldraw[magenta] (5.4,-0.95-0.15) circle (1.5pt);
    \draw[->,magenta] (5.4,-0.95-0.15) -- (6.6,-0.95-0.15);
    \draw[->,magenta] (5.4,-0.95-0.15) -- (6.6,0.65-0.15);
    \draw[->,magenta] (5.4,-0.95-0.15) -- (6.6,1.75-0.15);
    \draw[->,dashed] (5.2,-0.5-0.15) .. controls (5.8,-0.5-0.15) .. (6,-1.3-0.15);
    \node[] at (6,-1.7) {\scriptsize$\mathcal{N}_{s_p}$};

    
    \foreach \x/\y in {1.75/1,0.65/2,-0.95/m}
        \draw[fill=sage,rounded corners] (6.6,\x-0.15-0.3) rectangle node[black] {$a_\y$}++(0.5,0.5);
        %\node at (6.9,\x-0.15) {$a_\y$};
    \node at (6.9,-0.3) {$ \vdots$};
    % \foreach \x/\y in {0/1,1/2,2/3,3/4,5/Q-1,6/Q}
    %     \node at (8.4,2.25-0.617*\x-0.15) {$\phi_{\y}$};
    % \node at (8.4,-0.3) {$ \vdots$};

    % \draw[->] (7.2,1.6) -- (8.05,2.1);
    % \draw[->] (7.2,1.6) -- (8.05,1.48);
    
    % \draw[->] (7.2,0.5) -- (8.05,0.87);
    % \draw[->] (7.2,0.5) -- (8.05,0.25);
    
    % \draw[->] (7.2,-1.1) -- (8.05,-1.6);
    % \draw[->] (7.2,-1.1) -- (7.9,-0.98);
    % \draw[->,dashed] (7.4,1.3) ..controls (7.6,1.8) .. (7.3,1.97);
    % \node[] at (7.3,2.2) {\scriptsize$\mathcal{Q}_1$};
    % \draw[->,dashed] (7.4,-0.9) ..controls (7.65,-1.1) .. (7.5,-1.67) ;
    % \node[] at (7.5,-2) {\scriptsize$\mathcal{Q}_K$};
\end{tikzpicture}
% \caption{Network illustration of the described setting. Data assignment, followed by the Map, Shuffle and Reduce steps are depicted, with a symmetric task assignment, as $|\mathcal{Q}_1| = |\mathcal{Q}_2| = \ldots = |\mathcal{Q}_K| = 2$, meaning $Q = 2K$. Note that the transmissions from each node $k$ correspond to different values of $d_{q,k}X_k$. %For example, we can identify the transmissions from node 1 (the lines in dark blue) as $d_{3,1}X_1$, $d_{4,1}X_1$ to node 2 and $d_{Q-1,1}X_1, d_{Q,1}X_1$ to node K.
%}
\caption{WNCS Illustration (Not complete)}
\label{fig:network}
\end{figure}
